Well-posedness for the incompressible Hall-MHD system with initial magnetic field belonging to $H^{\frac{3}{2}}(\mathbb{R}^3)$

In this paper, we first prove the local well-posedness of strong solutions to the incompressible Hall-MHD system for initial data $(u_0,B_0)\in H^{\frac{1}{2}+\sigma}(\mathbb{R}^3)\times H^{\frac{3}{2}}(\mathbb{R}^3)$ with $\sigma\in (0,2)$. In particular, if the viscosity coefficient is equal to the resistivity coefficient, we can reduce $\sigma$ to $0$ with the aid of the new formulation of the Hall-MHD system observed by Danchin and Tan (Commun Partial Differ Equ 46(1):31-65, 2021). Compared with the previous works, our local well-posedness results improve the regularity condition on the initial data. Moreover, we establish the global well-posedness for small initial data in $H^{\frac{1}{2}+\sigma}(\mathbb{R}^3)\times H^{\frac{3}{2}}(\mathbb{R}^3)$ with $\sigma\in (0,2)$, and get the optimal time-decay rates of solutions.

==> _________ <==
that if in addition $(u_0,B_0)\in L^1(\mathbb{R}^3)$, the global small solutions of \eqref{main eq} in $H^m(\mathbb{R}^3)$ with $m\geq3$ satisfy\begin{equation}\label{cdecay}
	\|\nabla^ku(t)\|_{L^2}+\|\nabla^k B(t)\|_{L^2}\lesssim (1+t)^{-\frac{3}{4}-\frac{k}{2}}\quad\text{for}\quad 0\leq k\leq m.
\end{equation}

Later, Wan and Zhou in \cite{MR3397315} showed that if $(u_0,B_0)\in \dot{H}^{-s}(\mathbb{R}^3)$ with $0\leq s<\frac{3}{2}$, the following decay rate holds\begin{equation}
\|u(t)\|_{L^2}+\|B(t)\|_{L^2}\lesssim (1+t)^{-\frac{s}{2}},
\end{equation}and if $(u_0,B_0)\in \dot{B}^{-\frac{3}{2}}_{2,\infty}(\mathbb{R}^3)$, the decay estimate \eqref{cdecay} with $k=0$ holds. 

 $u_0$ is regular than $H^{\frac{1}{2}}(\mathbb{R}^3)$ as well as $B_0$ is regular than $H^{\frac{3}{2}}(\mathbb{R}^3)$.
 
 As mentioned above, the global existence and uniqueness of strong solutions to \eqref{main eq} with $\mu=\nu$ for small initial data $(u_0,B_0)\in \dot{H}^{\frac{1}{2}}(\mathbb{R}^3)\times (\dot{H}^{\frac{1}{2}}(\mathbb{R}^3)\cap \dot{H}^{\frac{3}{2}}(\mathbb{R}^3))$ was proved in \cite{MR4193644}. Although their initial data is less regular than that in \thmref{thm1}, their proof relies on \eqref{extend eq} and thus cannot be applied to the general case. To the best of our knowledge, there are no available global well-posedness result concerning \eqref{main eq} with $B_0\in H^{\frac{3}{2}}(\mathbb{R}^3)$ for the general $\mu$ and $\nu$, so it is significant to extend the local strong solutions constructed in \thmref{thm1} globally in time. We find that this can be achieved for small initial data. Furthermore, we obtain the optimal time-decay rates of solutions.
 
 we make no distinction between these two norms throughout this paper.
 
 
  in \lemref{prop}
  
  in \lemref{prop} 
  
  In order to avoid tracking the dependency of $\mu,\nu,\kappa$ for the constants in the proofs, we set $\mu=\nu=\kappa=1$ in the rest of this paper for the sake of simplicity. 
  
  and follow the same process leading to \eqref{apriores}, we can deduce that for all $t\in [0,T_n)$,
  
  where the constant $L>0$ depends on the norm of $(u_0,B_0)$.
  
  \\
  &\leq 2C_1(\|u_0\|_{{H}^{\frac{1}{2}+\sigma}}+\|B_0\|_{{H}^{\frac{3}{2}}}).
  
  On the other hand, remember that $B\in C([0,T_*];H^{s_2})$ with $s_2<\frac{3}{2}$ and $B\in L^\infty(0,T_*;H^{\frac{3}{2}})$, since $H^{-s_2}$ is dense in $H^{-\frac{3}{2}}$, by means of an $\frac{\epsilon}{2}$-argument, it is easy to show that $B$ is continuous in the weak topology of $H^{\frac{3}{2}}$ with respect to time, which implies that\begin{equation}
  \varliminf _{t\rightarrow 0^+}\|B(t)\|_{H^{\frac{3}{2}}}\geq \|B_0\|_{H^{\frac{3}{2}}}.
  \end{equation}
  
  In constrast to the time-decay estimates in \cite{MR3097244,MR3397315}, since $L^1(\mathbb{R}^3)\cap L^2(\mathbb{R}^3)\hookrightarrow \dot{H}^{-\gamma}(\mathbb{R}^3)\hookrightarrow \dot{B}^{-\gamma}_{2,\infty}(\mathbb{R}^3)$ for $ \gamma\in[0,\frac{3}{2}]$, we relax the regularity condition on the initial data and expand the range of $\gamma$ from $[0,\frac{3}{2}]$ to $[0,\frac{5}{2}]$.
  
  However, in the $\dot{H}^r$-estimates of the magnetic equation, by and ,  the usual treament for the Hall term formally give us
  
  However, the usual treament for the Hall term formally give us
  
  For the less regular initial data in Sobolev spaces, the local well-posedness of \eqref{main eq} in $H^s(\mathbb{R}^3)\times H^s(\mathbb{R}^3)$ with $s=2$ was proved by Benvenutti and Ferreira \cite{MR3513590}, with $s>\frac{3}{2}$ was proved by Dai \cite{MR4060362} and with $\frac{3}{2}<s\leq\frac{5}{2}$ was obtained in \cite{MR3770153}. 
  
  \\
  &\leq 2C_1(\|u_0\|_{{H}^{\frac{1}{2}+\sigma}}+\|B_0\|_{{H}^{\frac{3}{2}}})
  
  \\&\leq C(\|u_0\|_{{H}^{\frac{1}{2}+\sigma}},\|B_0\|_{{H}^{\frac{3}{2}}})
  
  where $T_*$ and $M$ only depend on the norm of initial data.
  
  the initial magnetic field 
  
  From the previous section, we see that the core of the proof of \thmref{thm1} is to establish the uniform bounds for the approximate solutions. In what follows, we only show how to use \eqref{extend eq} to derive the desired bound of smooth solutions on a short time interval $[0,T_*]$, the remainder of the proof of \thmref{thm2} can be proceed in a same way as in the previous section and thus is omitted.\par 
  
  where $T_*$ and $M$ are uniform with respect to all approximate solutions.
  
  We should point out that all previous results on the local well-posedness for \eqref{main eq} in nonhomogeneous Sobolev spaces require $(u_0,B_0)\in H^{s}(\mathbb{R}^3)\times H^{r}(\mathbb{R}^3)$ with some $s>\frac{1}{2}$ and $r>\frac{3}{2}$. 
  
  Our results improves some previous works. 
  
  Compared with previous works, our results allow initial magnetic field $B_0$ to belong to $H^{\frac{3}{2}}(\mathbb{R}^3)$.
  
  By ultilizing \eqref{extend eq}, we indeed can reduce $\sigma$ in \thmref{thm1} to $0$  in the special case $\mu=\nu$. 
  
   when considering \eqref{extend eq}
   
   for the special case $\mu=\nu$
   
   For the less regular initial data in Sobolev spaces, the local well-posedness of \eqref{main eq} in $H^s(\mathbb{R}^3)\times H^s(\mathbb{R}^3)$ with $s=2$ was proved by Benvenutti and Ferreira \cite{MR3513590}, with $s>\frac{3}{2}$ was proved by Dai \cite{MR4060362} and with $\frac{3}{2}<s\leq\frac{5}{2}$ was obtained in \cite{MR3770153}. 
   
   Recently, Dai \cite{MR4248458} proved that \eqref{main eq} is locally well-posed in $H^{s-1+\sigma}(\mathbb{R}^3)\times H^s(\mathbb{R}^3)$ with $s>\frac{3}{2}$ and $\sigma>0$. 
   
   Dai \cite{MR4248458} proved the local well-posedness of \eqref{main eq} in $H^{s-1+\sigma}(\mathbb{R}^3)\times H^s(\mathbb{R}^3)$ with $s>\frac{3}{2}$ and $\sigma>0$.
   
   treat the Hall term as\begin{equation}\begin{split}
   \Big(\Lambda^r \nabla\times(B\times(\nabla\times B)),\Lambda^r B\Big)&\lesssim\|[\Lambda^{r},B\times](\nabla\times B)\|_{L^2}\|B\|_{\dot{H}^{r+1}}\\
   &\lesssim\|\Lambda^{r}B\|_{L^{p_1}}\|\nabla B\|_{L^{p_2}}\|B\|_{\dot{H}^{r+1}}\\
   &\lesssim\|B\|_{\dot{H}^{r+\frac{3}{p_2}}}\|B\|_{\dot{H}^{1+\frac{3}{p_1}}}\|B\|_{\dot{H}^{r+1}}\\
   &\lesssim \Big(\|B\|_{\dot{H}^{r}}^{1-\frac{3}{p_2}}\|B\|_{\dot{H}^{r+1}}^{\frac{3}{p_2}}\Big)\Big(\|B\|_{\dot{H}^{r}}^{r-\frac{3}{p_1}}\|B\|_{\dot{H}^{r+1}}^{\frac{3}{p_1}+1-r}\Big)\|B\|_{\dot{H}^{r+1}}\\
   &\lesssim \|B\|_{\dot{H}^{r}}^{r-\frac{1}{2}}\|B\|_{\dot{H}^{r+1}}^{\frac{7}{2}-r}
   \end{split}
   \end{equation}
   
   thus this method may not work in the case of $B_0\in H^{\frac{3}{2}}(\mathbb{R}^3)$.
   
   $H^{s-1+\sigma}(\mathbb{R}^3)\times H^s(\mathbb{R}^3)$
   
   \quad\text{for all}\quad t\geq 0, 
   
   	Let $\gamma\in[0,\frac{5}{2}]$ and $(u_0,B_0)\in \dot{B}^{-\gamma}_{2,\infty}(\mathbb{R}^3)$, it holds that for all $t\geq 0$,\begin{equation}\label{nbound}
   \|u(t)\|_{\dot{B}^{-\gamma}_{2,\infty}}+\|B(t)\|_{\dot{B}^{-\gamma}_{2,\infty}}\leq C_0,
   \end{equation}where $C_0$ is a positive constant and depends on the norms of the initial data.
   
   Therefore, it seems hard to reduce $\sigma$ to $0$ in \thmref{thm1} for the time being.
   
   prove the local well-posedness of \eqref{main eq} in $H^{\frac{1}{2}}(\mathbb{R}^3)\times H^{\frac{3}{2}}(\mathbb{R}^3)$
   
   \textsc{School of Mathematical Sciences, Shanghai Jiao Tong University, Shanghai 200240, P.R.China}\par 
   E-mail address: zhangshunhang@sjtu.edu.cn
   
   the initial magetic field 
   
   Let $s_1,s_2\in\mathbb{R}$ and $1\leq p,p_1,p_2,r,r_1,r_2\leq\infty$ with $\frac{1}{p}=\frac{1}{p_1}+\frac{1}{p_2}$ and $\frac{1}{r}\leq \frac{1}{r_1}+\frac{1}{r_2}$. If $s_1+s_2>0$, there exists a constant $C$ such that\begin{equation}
   \begin{split}
   \|\dot{R}(u,v)\|_{\dot{B}^{s_1+s_2}_{p,r}}\leq C\|u\|_{\dot{B}^{s_1}_{p_1,r_1}}\|v\|_{\dot{B}^{s_2}_{p_2,r_2}}.
   \end{split}
   \end{equation}If $r=1$ and $s_1+s_2=0$, there exists a constant $C$ such that\begin{equation}\label{zero}
   \begin{split}
   \|\dot{R}(u,v)\|_{\dot{B}^{0}_{p,\infty}}\leq C\|u\|_{\dot{B}^{s_1}_{p_1,r_1}}\|v\|_{\dot{B}^{s_2}_{p_2,r_2}}.
   \end{split}
   \end{equation}
   
   $(u,B)\in H^s\times H^s$ 
   
   \quad\text{for all}\quad t\geq 0
   
   for all $t\geq 0$ 
   
   $(u_0,B_0)\in H^{\frac{1}{2}+\sigma}(\mathbb{R}^3)\times H^{\frac{3}{2}}(\mathbb{R}^3)$
   
   \begin{lem}[\cite{MR2768550}]\label{product1}
   Let $s\in\mathbb{R}$, $t<0$ and $1\leq p,r\leq\infty$, there exists a constant $C$ such that
   \begin{equation}
   \begin{split}
   \|\dot{T}_uv\|_{\dot{B}^{s}_{p,r}}&\leq C \|u\|_{{L^{\infty}}}\|v\|_{\dot{B}^{s}_{p,r}}\quad\text{and}\quad\|\dot{T}_uv\|_{\dot{B}^{s+t}_{p,r}}\leq C\|u\|_{\dot{B}^{t}_{\infty,\infty}}\|v\|_{\dot{B}^{s}_{p,r}}.
   \end{split}
   \end{equation}
   Let $s_1,s_2\in\mathbb{R}$ and $1\leq p,p_1,p_2,r,r_1,r_2\leq\infty$ with $\frac{1}{p}=\frac{1}{p_1}+\frac{1}{p_2}$ and $\frac{1}{r}\leq \frac{1}{r_1}+\frac{1}{r_2}$. If $s_1+s_2>0$, there exists a constant $C$ such that\begin{equation}
   \begin{split}
   \|\dot{R}(u,v)\|_{\dot{B}^{s_1+s_2}_{p,r}}\leq C\|u\|_{\dot{B}^{s_1}_{p_1,r_1}}\|v\|_{\dot{B}^{s_2}_{p_2,r_2}}.
   \end{split}
   \end{equation}If $r=1$ and $s_1+s_2=0$, there exists a constant $C$ such that\begin{equation}\label{zero}
   \begin{split}
   \|\dot{R}(u,v)\|_{\dot{B}^{0}_{p,\infty}}\leq C\|u\|_{\dot{B}^{s_1}_{p_1,r_1}}\|v\|_{\dot{B}^{s_2}_{p_2,r_2}}.
   \end{split}
   \end{equation}
   \end{lem}
   
   Let $s_1,s_2\in\mathbb{R}$ and $1\leq p,p_1,p_2,r,r_1,r_2\leq\infty$ satisfying $s_1+s_2>0$, $\frac{1}{p}=\frac{1}{p_1}+\frac{1}{p_2}$ and $\frac{1}{r}=\frac{1}{r_1}+\frac{1}{r_2}$, there exists a constant $C$ such that
